Critical dynamics of relativistic diffusion

We study the dynamics of self-interacting scalar fields with $Z_2$ symmetry governed by a relativistic Israel-Stuart type diffusion equation in the vicinity of a critical point. We calculate spectral functions of the order parameter in mean-field approximation as well as using first-principles classical-statistical lattice simulations in real-time. We observe that the spectral functions are well-described by single Breit-Wigner shapes. Away from criticality, the dispersion matches the expectations from the mean-field approach. At the critical point, the spectral functions largely keep their Breit-Wigner shape, albeit with non-trivial power-law dispersion relations. We extract the characteristic time-scales as well as the dynamic critical exponent $z$, verifying the existence of a dynamic scaling regime. In addition, we derive the universal scaling functions implied by the Breit-Wigner shape with critical power-law dispersion and show that they match the data. Considering equations of motion for a system coupled to a heat bath as well as an isolated system, we perform this study for two different dynamic universality classes, both in two and three spatial dimensions.

==> tables/amp.tex <==
& $z(\gamma=1.0)$& $f_t(\gamma=1.0)$& $z(\gamma=0.1)$& $f_t(\gamma=0.1)$& $z(\gamma=0.0)$& $f_t(\gamma=0.0)$\\ \hline
2D & 3.83(10)& 1.04(14)& 3.716(17)& 0.190(8)& 2.354(23)& 0.358(19)\\
3D & 3.95(8)& 0.73(6)& 3.91(6)& 0.090(10)& 2.20(13)& 0.14(5)


==> tables/bwfit.tex <==
& $z_{\omega}$& $\omega^2_0$& $z_{\Gamma}$& $\Gamma_0$\\ \hline
2D & 3.769(13)& 1.81(6)& 1.612(21)& 1.29(7)\\
3D & 3.9660(20)& 1.3430(25)& 1.43(6)& 0.059(9)\\


==> vertices.tex <==
\section{Four-point vertex for \tops{$a=2$}{a=2}}\label{app:vertex}
We define the Fourier transformation as
\begin{align}
    \tphi(\vk) = \int \intd^d x \phi(\vx) e^{-\iu\vk \vx},\quad
    \phi(\vx) = \int \frac{\intd^d k}{(2\pi)^d} \tphi(\vk) e^{\iu\vk \vx},
\end{align}
for the field and analogous for the conjugate momentum $\pi$.
%The variational/partial derivatives become
%\begin{align}
%    \frac{\delta \tphi(\vk)}{\delta\phi(\vx)} = e^{-\iu\vk\vx},\quad
%    \frac{\delta \phi(\vx)}{\delta\tphi(\vk)} = e^{\iu\vk\vx},
%\end{align}
%which necessitates the absorbption of the factor $(2\pi)^d$ into $\delta/\delta \tphi(\vk)$ to not introduce inconsistencies.

We now want to find a Hamiltonian $H'_B[\pi,\phi]$ (compare \cref{eq:H2prime}) with canonically conjugate fields $\phi, \pi\equiv\dot \phi$ that generates the conservative part of the equations of motion \cref{eq:ModelB_eom}.
These equations of motion contain a non-local interaction term of the form
\begin{equation}
    \frac{\delta}{\delta\phi(x)} H'_B = 4\nabla^2 \phi(x)^3 = \int \intd^dk \; \intd^{d} \intd k_1\; \intd^d k_2\;  \vk^2 \phi(\vk_1)\phi(\vk_2)\phi(-\vk-\vk_1-\vk_2) e^{\iu \vk \vx}.
\end{equation}
To find $H'_B$, we start with the following ansatz, which is a generalization of the local four-point interaction vertex:
\begin{equation}
    H'_B = \int \intd^dk \;\intd^dk_1\;\intd^dk_2\;f\left( \vk,\vk_1,\vk_2 \right)\tphi(\vk)\tphi(\vk_1)\tphi(\vk_2)\tphi(-\vk-\vk_1-\vk_2),
\end{equation}
where $f(\vk,\vk_1,\vk_2)$ is a scalar function of the momenta.
Variation w.r.t.~$\tphi(\vk)$ yields the defining equation for $f(\vk, \vk_1, \vk_2)$ as
\begin{align}
    \vk^{2} &\seq f(\vk,\vk_1,\vk_2) + f(-\vk-\vk_1-\vk_2,\vk_1,\vk_2) + f(\vk_1,\vk,\vk_2) + f(\vk_2,\vk_1,\vk),\\
    \follows f\left( \vk,\vk_1,\vk_2 \right) &= \frac{\vk^4}{2\left( \vk^2 + \vk\vk_1 + \vk\vk_2 + \vk_1^2 + \vk_1\vk_2 + \vk_2^2 \right)} \\
    &= \frac{\vk^4}{\vk^2 + \vk_1^2 + \vk_2^2 + \left( \vk+\vk_1+\vk_2 \right)^2},
\end{align}
whereby we find for the interaction term
\begin{equation}
    H'_B = \int \intd^dk \;\intd^dk_1\;\intd^dk_2\; \frac{\vk^4 \tphi(\vk)\tphi(\vk_1)\tphi(\vk_2)\tphi(-\vk-\vk_1-\vk_2)}{\vk^2 + \vk_1^2 + \vk_2^2 + (\vk+\vk_1+\vk_2)^2}.
    \label{eq:modelb_HI_k}
\end{equation}
At this point, we have not attempted to derive the equivalent expression in coordinate space.

